DTMamba : Dual Twin Mamba for Time Series Forecasting

We utilized the Mamba model for time series data prediction tasks, and the experimental results indicate that our model performs well.

==> head.bak.tex <==
%%%%%% !TEX root = mamba.tex

%\special{papersize=210mm,297mm}% a4paper
%\pdfpagewidth 210mm
%\pdfpageheight 297mm

%\special{papersize=8.5in,11in}% letter paper
%\pdfpagewidth 8.5in
%\pdfpageheight 11.0in

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% for vldbj cls
%\usepackage[margin=0.1in]{geometry}
%
% for sig cls
% tweak page size and offsets during development
% TODO: remove before submission
%  \pdfpagewidth=7.2in
%  \pdfpageheight=9.5in
%  \hoffset=-0.65in
%  \voffset=-0.65in
%  \special{papersize=185mm,240mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% section --------------------------------------------
\makeatletter %
\let\proof\@undefined
\let\endproof\@undefined
%
%\renewcommand\subsubsection{\@startsection{paragraph}{4}{\z@}{3\p@ \@plus \p@}{-5\p@}{\normalsize\bfseries}}
%\@ifundefined{abovecaptionskip}{
% \newskip\abovecaptionskip \abovecaptionskip=0em
% \newskip\belowcaptionskip \belowcaptionskip=0em
% \long\def\@makecaption#1#2{%
%   \vskip\abovecaptionskip
%   \setbox\@tempboxa\hbox{\textbf{#1: #2}}
%   \ifdim \wd\@tempboxa >\hsize % IF longer than one line:
%       \textbf{#1: #2}\par      %   THEN set as ordinary paragraph.
%     \else                      %   ELSE  center.
%       \hbox to\hsize{\hfil\box\@tempboxa\hfil}\par
%   \fi
%   \vskip\belowcaptionskip
%   }%
%}{} %
%
%\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}{3\p@ \@plus \p@}{-5\p@}{\normalsize\itshape}}
%\@ifundefined{abovecaptionskip}{
% \newskip\abovecaptionskip \abovecaptionskip=0em
% \newskip\belowcaptionskip \belowcaptionskip=0em
% \long\def\@makecaption#1#2{%
%   \vskip\abovecaptionskip
%   \setbox\@tempboxa\hbox{\textbf{#1: #2}}
%   \ifdim \wd\@tempboxa >\hsize % IF longer than one line:
%       \textbf{#1: #2}\par      %   THEN set as ordinary paragraph.
%     \else                      %   ELSE  center.
%       \hbox to\hsize{\hfil\box\@tempboxa\hfil}\par
%   \fi
%   \vskip\belowcaptionskip
%   }%
%}{} %%
%
% enumerate format
%\renewcommand{\labelenumi}{(\arabic{enumi})}
%\renewenvironment{enumerate}{ %	%%%% Begin preliminary environment code
%	\begin{list}{ %		%%%% Begin list item label code
%		%\bfseries\upshape\arabic{enumi}:
%      \labelenumi
%	}{ %	%%%% Begin list item body code
%		\usecounter{enumi}
%		%\setlength{\labelwidth}{1in}
%		\setlength{\leftmargin}{0in}
%		\setlength{\itemindent}{2em} % or 0em
%		\setlength{\itemsep}{0em}
%		%\setlength{\parsep}{0ex}
%	} %%%%% End list item body code
%}{ %%%%% Begin wrapup environment code
%	\end{list}
%}  %%%%% End wrapup environment code
%
\makeatother %

% tight drafting
%\setlength{\headheight}{-5pt}
%\setlength{\headsep}{0pt}
%\setlength{\hoffset}{-45pt}
%\special{papersize=7.5in,9.5in}


% package --------------------------------------------
%\usepackage[letterpaper]{geometry}
\usepackage{color}
%\usepackage{times}
\let\Bbbk\relax         %%redefined in newtxmath.sty
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amsfonts}
%\usepackage[boxed]{algorithm}
%\usepackage[ruled]{algorithm}
%\usepackage{algorithmic}
%\usepackage[noend]{algorithmic}
\usepackage[ruled,noend,linesnumbered]{algorithm2e}
\usepackage{balance}
\usepackage{textcomp}%\texttildelow
\usepackage{url}%~
\usepackage{enumitem} % conflict with IEEEtran
\usepackage{comment}
\usepackage[labelfont=bf]{caption} %font=small,

% proof --------------------------------------------
%\makeatletter
%\renewenvironment{proof}[1][\proofname]{\par
%% \vspace{-\topsep}% remove the space after the theorem
%  \pushQED{\qed}%
%  \normalfont \partopsep=\z@skip \topsep=\z@skip
%  \trivlist
%  \item[\hskip\labelsep
%        \itshape
%    #1\@addpunct{.}]\ignorespaces
%}{%
%  \popQED\endtrivlist\@endpefalse
%%  \addvspace{6pt plus 6pt} % some space after
%}
%\renewcommand{\labelenumi}{\arabic{enumi}. }
%\makeatother

% space --------------------------------------------
%\usepackage[font=footnotesize,bf,up]{caption}
%\captionsetup[table]{labelfont=small}%

%\setlength{\abovecaptionskip}{0em} % Space above float caption
%\setlength{\belowcaptionskip}{0em} % Space below float caption

%\setlength{\intextsep}{0em} %Space above and below in-line text floats
%\setlength{\intextsep}{0.5em plus 2pt minus 2pt} 

%\setlength{\topsep}{0em} %theorem
%\setlength{\parsep}{0em} %Paragraph separation within a single item.
%\setlength{\partopsep}{0em} %proof

%\setlength{\floatsep}{0em} %Space between floats. \dblfloatsep for 2 column format
%\setlength{\textfloatsep}{0em} %space between last top float or first bottom float and the text.

%\setlength{\abovedisplayskip}{0em} %space before maths
%\setlength{\belowdisplayskip}{0em} %space after maths

% environment ----------------------------------------
\newlength{\figwidths}
\setlength{\figwidths}{3in}
\newlength{\figwidthd}
\setlength{\figwidthd}{4.1in}
\newlength{\expwidths}
\setlength{\expwidths}{3.6in}
\newlength{\expwidthd}
\setlength{\expwidthd}{7.2in}

\theoremstyle{plain}% default
\newtheorem{definitions}{Definition}%[section]
\newtheorem{problems}{Problem}%[section]
\newtheorem{theorems}{Theorem}%[section]
\newtheorem{lemmas}[theorems]{Lemma}%[section]
\newtheorem{claims}[theorems]{Claim}%[section]
\newtheorem{corollaries}[theorems]{Corollary}%[section]
\newtheorem{propositions}[theorems]{Proposition}%[section]

\makeatletter  
\def\@endtheorem{\hfill\ensuremath{\blacksquare}\endtrivlist\@endpefalse } % insert `\qed` macro
\makeatother
\theoremstyle{definition}
\newtheorem{examples}{Example}%[section]

\theoremstyle{remark}
\newtheorem*{remarks}{Remark}
\newtheorem*{notes}{Note}
\newtheorem{case}{Case}
\newtheorem*{proofs}{Proof sketch}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}

%% revision --------------------------------------------
%\makeatletter
%\newenvironment{questions}[1][Q]{\par
%\addvspace{6pt plus 6pt}% \vspace{-\topsep}% remove the space after the theorem
%%\pushQED{\qed}%
%  \fontsize{10pt}{1.5em}
%  \normalfont \partopsep=\z@skip \topsep=\z@skip
%  \trivlist
%  \item[\hskip\labelsep
%        \bfseries
%    #1\@addpunct{:}]\ignorespaces
%    \itshape\color{blue}
%}{%
%%  \popQED
%\endtrivlist\@endpefalse
%%  \addvspace{6pt plus 6pt} % some space after
%}
%\newenvironment{reply}[1][Reply]{\par
%\addvspace{3pt plus 3pt}% \vspace{-\topsep}% remove the space after the theorem
%  \pushQED{\qed}%
%  \fontsize{10pt}{1.5em}
%  \normalfont \partopsep=\z@skip \topsep=\z@skip
%  \trivlist
%  \item[\hskip\labelsep
%        \scshape
%    #1\@addpunct{:}]\ignorespaces
%}{%
%  \popQED\endtrivlist\@endpefalse
%%  \addvspace{6pt plus 6pt} % some space after
%}
%\newenvironment{summary}{\par
%\addvspace{3pt plus 3pt}% \vspace{-\topsep}% remove the space after the theorem
%  \fontsize{10pt}{1.5em}
%  \normalfont \partopsep=\z@skip \topsep=\z@skip
%}{%
%%  \addvspace{6pt plus 6pt} % some space after
%}
%\newenvironment{revised}{\color{blue}}
%\makeatother

% general ---------------------------------------------
\newcommand{\comments}{\textcolor{red}}
\newcommand{\zaq}{\textcolor{magenta}}
\newcommand{\wzx}{\textcolor{purple}}
\newcommand{\nop}[1]{}
\newcommand{\na}{\textsc{n/a}}
\newcommand{\lhs}{\textsc{lhs}}
\newcommand{\rhs}{\textsc{rhs}}

\newcommand{\p}{\textsc{p}}
\newcommand{\ptime}{\textsc{ptime}}
\newcommand{\np}{\textsc{np}}
\newcommand{\npc}{\textsc{np}-complete}
\newcommand{\nph}{\textsc{np}-hard}

% dependency ---------------------------------------------
\newcommand{\eqc}{\textsc{eqc}}
\newcommand{\eqcs}{\textsc{eqc}s}

\newcommand{\mdc}{\textsc{mdc}}
\newcommand{\mdcs}{\textsc{mdc}s}

\newcommand{\ind}{\textsc{ind}}
\newcommand{\inds}{\textsc{ind}s}

\newcommand{\fd}{\textsc{fd}}
\newcommand{\fds}{\textsc{fd}s}
\newcommand{\cfd}{\textsc{cfd}}
\newcommand{\cfds}{\textsc{cfd}s}

\newcommand{\cd}{\textsc{cd}}
\newcommand{\cds}{\textsc{cd}s}

\newcommand{\md}{\textsc{md}}
\newcommand{\mds}{\textsc{md}s}

\newcommand{\mfd}{\textsc{mfd}}
\newcommand{\mfds}{\textsc{mfd}s}

\newcommand{\od}{\textsc{od}}
\newcommand{\ods}{\textsc{od}s}

\newcommand{\sd}{\textsc{sd}}
\newcommand{\sds}{\textsc{sd}s}
\newcommand{\csd}{\textsc{csd}}
\newcommand{\csds}{\textsc{csd}s}

\newcommand{\dd}{\textsc{dd}}
\newcommand{\dds}{\textsc{dd}s}
\newcommand{\DDs}{DDs}
\newcommand{\cdk}{\textsc{cdk}}
\newcommand{\cdks}{\textsc{cdk}s}
\newcommand{\CDKs}{CDKs}

% local ---------------------------------------------


